Direct visualization of electronic transport in a quantum anomalous Hall insulator

A quantum anomalous Hall (QAH) insulator is characterized by quantized Hall and vanishing longitudinal resistances at zero magnetic field that are protected against local perturbations and independent of sample details. This insensitivity makes the microscopic details of the local current distribution inaccessible to global transport measurements. Accordingly, the current distributions that give rise to the transport quantization are unknown. Here we use magnetic imaging to directly visualize the transport current in the QAH regime. As we tune through the QAH plateau by electrostatic gating, we clearly identify a regime in which the sample transports current primarily in the bulk rather than along the edges. Furthermore, we image the local response of the magnetization to electrostatic gating. Combined, these measurements suggest that incompressible regions carry the current within the QAH regime. Our observations indicate that the self-consistent electrostatics of the sample play a central role in determining the current distribution. Identifying the appropriate microscopic picture of electronic transport in QAH insulators and other topologically non-trivial states of matter is a crucial step towards realizing their potential in next-generation quantum devices.

==> Recycle_bin.tex <==
Instead, we find that a dissipationless Hall current driven by transverse electric fields dominates transport in our devices.


that interplay between Fermi level pinning and the unusual transport properties of materials with a high hall angle results in





\section{Supplement} 

\subsection{Device fabrication}:


\subsection{Measurements outside the gap}:

\subsection{Magnetization dependence}: Here we present complementary data to the data in the sample with the magnetization direction reversed.

\subsection{Linear response}:

\subsection{Imaging protocols}: 

\subsection{Measurements on a second device}: In addition to the data collected on the Hall bar, we measured a second two-terminal device fabricated on the same chip. We observe a qualitatively similar behavior between both devices. 



%We speculate that \dMdV originates from two dominant mechanisms (see SI for details). Both tend to reduce the magnetization as $\mu$ increases consistent with our measurements. First, the charge carriers in the device contribute an orbital magnetization $M_{orb}$ that depends on the band filling and the distribution of Berry curvature within the conduction and valence bands[CITE Niu review]. Second, the addition and removal of itinerant electrons may modify the strength of the exchange coupling between the Cr dopants, leading to a change in the magnetization of the dopant atoms $M_{\mathrm{Cr}}$. When $\mu$ is in the gap, $dM_{\mathrm{orb}}/dV$ is expected to be maximal and given by $\sigma_{xy} * d\mu/d(eV_{TG})$ [CITE Streda?]. The maximum amplitude in our data is approximately 2\% of $\sigma_{xy}$, which suggests that localized mid-gap states limit the efficiency with which the top gate can modulate the chemical potential. Several studies of Cr-doped (BiSb)$_2$Te$_3$ indicate that a hole-mediated RKKY coupling contributes to the exchange coupling between Cr dopants. The strength of the exchange coupling therefore depends on the valence band filling [CITE]. In this case, $dM_{Cr}/dV$ is expected to be finite when $\mu$ is in the valence band and negligible when $\mu$ is either in the gap or conduction band. However, no estimate for the strength of $dM_{Cr}/dV$ is available. $dM_{Cr}/dV$ is only bounded by the requirement that $M$ remains finite when $\mu$ reaches the gap. The measured \dMdV has a significantly different magnitude for $\mu$ in the conduction and valence band, which is consistent with the above mechanisms. In addition, we observe a shallow minimum as a function of $V_{BG}$, which is reminiscent of the expected plateau when $\mu$ is in the gap. Clarifying the amplitude of \dMdV, the detailed spatial and $V_{BG}$ dependence and the role of additional mechanisms will be explored in further work. Regardless, \dMdV shown in Fig. 3g provides us with knowledge of how $\mu$ locally crosses from the valence band into the conduction band. 


%where the local maximum in \dMdV first emerges in the center of the channel (Fig. 3i), $\sigma_{xy}$ rapidly increases towards $e^2/h$. As the decrease in the magnitude of \dMdV spreads over the channel, $\sigma_{xy}$ remains unchanged and quantized. However, once it reaches the edges of the channel near $V_{\mathrm{BG}} = 150 V$, $\sigma_{xy}$ begins to decreases again.


%To compare this picture to our results we use \dMdV to constrain the spatial structure of the incompressible regions in which $\mu$ is in the gap. For each position along $y$, we find the range of $V_{\mathrm{BG}}$ in which \dMdV is transitioning (Fig. 4a), indicating that the chemical potential is locally tuned through the gap. To compare the structure of these regions to the current distribution, we normalize the current density $j_x$ from Fig. 3d using $j_{rn} = j_y / (\max \{j_y\} - \min \{j_y\})$ to highlight the locations of the sample that support a finite current density (Fig. 4b). The bifurcation in the current density as the sample is tuned through the QAH regime is clearly visible. We plot the data as a function of $V_{\mathrm{BG}}-V_{Gap}$, where $V_{Gap}$ is the back gate voltage that maximizes $R_{xy}$ (see SI for details). Small shifts in $V_{Gap}$ between individual gate sweeps likely arises from a well-documented charging effect in STO gated devices \cite{serlin2020intrinsic, biscaras2014limit, mikheev2020quantized}. Remarkably, we find that the positions of high current density closely track the regions that we identify as incompressible in the \dMdV measurement.

%So far we have not addressed the motion of the incompressible strips under an applied bias current or top gate excitation. When the sample is biased with an external current, the potential landscape in the channel changes, effectively gating the sample and shifting the position of the incompressible strips. Given that the incompressible strips carry an equilibrium current, their motion may generate an additional contribution to the current density. This bias induced gating is difficult to disentangle from the externally biased transport current. A fully self-consistent electrostatic solution for the position and motion of the incompressible strips under an external bias current is required to fully reproduce all features of the data. For example, motion of these incompressible strips under an applied bias can account for the backwards flowing current that we observe in Figs. 2e and 4b (see SI for details).

%The model for conduction outlined above does not account for the motion of the incompressible strips under an applied bias current or top gate excitation. For example, we observe a counter flowing current at the bottom edge of the device at each back gate voltage (Fig. 4b) that can be understood as bias-driven motion of the current-carrying incompressible strip (See supplement for details). Although beyond the scope of this work, we anticipate that a fully self-consistent electrostatic solution for the position and motion of the incompressible strips will allow us to reproduce the observed current distributions in detail. 

==> authors.tex <==
\title{Direct visualization of electronic transport in a quantum anomalous Hall insulator}
\author{G. M. Ferguson}\affiliation{Laboratory of Atomic and Solid-State Physics, Cornell University, Ithaca, NY 14853, USA} 
\author{Run Xiao}\affiliation{Department of Physics, The Pennsylvania State University, University Park, 16802, Pennsylvania, USA}
\author{Anthony R. Richardella}\affiliation{Department of Physics, The Pennsylvania State University, University Park, 16802, Pennsylvania, USA}
\author{David Low}\affiliation{Laboratory of Atomic and Solid-State Physics, Cornell University, Ithaca, NY 14853, USA}
\author{Nitin Samarth}\affiliation{Department of Physics, The Pennsylvania State University, University Park, 16802, Pennsylvania, USA}
\author{Katja C. Nowack}\email{kcn34@cornell.edu}\affiliation{Laboratory of Atomic and Solid-State Physics, Cornell University, Ithaca, NY 14853, USA}\affiliation{Kavli Institute at Cornell for Nanoscale Science, Cornell University, Ithaca, NY 14853, USA}
